Modeling social interaction dynamics using temporal graph networks

Integrating intelligent systems, such as robots, into dynamic group settings poses challenges due to the mutual influence of human behaviors and internal states. A robust representation of social interaction dynamics is essential for effective human-robot collaboration. Existing approaches often narrow their focus to facial expressions or speech, overlooking the broader context. We propose employing an adapted Temporal Graph Networks to comprehensively represent social interaction dynamics while enabling its practical implementation. Our method incorporates temporal multi-modal behavioral data including gaze interaction, voice activity and environmental context. This representation of social interaction dynamics is trained as a link prediction problem using annotated gaze interaction data. The F1-score outperformed the baseline model by 37.0%. This improvement is consistent for a secondary task of next speaker prediction which achieves an improvement of 29.0%. Our contributions are two-fold, including a model to representing social interaction dynamics which can be used for many downstream human-robot interaction tasks like human state inference and next speaker prediction. More importantly, this is achieved using a more concise yet efficient message passing method, significantly reducing it from 768 to 14 elements, while outperforming the baseline model.

==> keywords.tex <==
priority 1, 2, 3

Affective Computing
Androids
Anthropomorphic Robots and Virtual Humans
Applications of Social Robots
Art pieces supported by robotics
Assistive Robotics
Child-Robot Interaction
Cognitive Skills and Mental Models
Cognitive and Sensorimotor Development
Computational Architectures
Cooperation and Collaboration in Human-Robot Teams
Creating Human-Robot Relationships
Curiosity, Intentionality and Initiative in Interaction
Degrees of Autonomy and Teleoperation
Detecting and Understanding Human Activity
Embodiment, Empathy and Intersubjectivity
Ethical Issues in Human-robot Interaction Research
Evaluation Methods
HRI and Collaboration in Manufacturing Environments
Human Factors and Ergonomics
Innovative Robot Designs
Interaction Kinesics
Interaction with Believable Characters
Linguistic Communication and Dialogue
Long-term Experience and Longitudinal HRI Studies
Machine Learning and Adaptation
Medical and Surgical Applications
\textbf{Monitoring of Behaviour and Internal States of Humans}
Motion Planning and Navigation in Human-Centered Environments
Motivations and Emotions in Robotics
Multi-modal Situation Awareness and Spatial Cognition
Multimodal Interaction and Conversational Skills
Narrative and Story-telling in Interaction
\textbf{Non-verbal Cues and Expressiveness}
Novel Interfaces and Interaction Modalities
Personalities for Robotic or Virtual Characters
Philosophical Issues in Human-Robot Coexistence
Programming by Demonstration
Robot Companions and Social Robots
Robotic Etiquette
Robots in Education, Therapy and Rehabilitation
Robots in art and entertainment
\textbf{Social Intelligence for Robots}
Social Learning and Skill Acquisition Via Teaching and Imitation
Social Presence for Robots and Virtual Humans
Social Touch in Human–Robot Interaction
Sound design for robots
Storytelling in HRI
User-centered Design of Robots
Virtual and Augmented Tele-presence Environments
